Towards Video Codec Performance Evaluation: A Rate-Energy-Distortion Perspective

The Bj{\o}ntegaard Delta rate (BD-rate) objectively assesses the coding efficiency of video codecs using the rate-distortion (R-D) performance but overlooks encoding energy, which is crucial in practical applications, especially for those on handheld devices. Although R-D analysis can be extended to incorporate encoding energy as energy-distortion (E-D), it fails to integrate all three parameters seamlessly. This work proposes a novel approach to address this limitation by introducing a 3D representation of rate, encoding energy, and distortion through surface fitting. In addition, we evaluate various surface fitting techniques based on their accuracy and investigate the proposed 3D representation and its projections. The overlapping areas in projections help in encoder selection and recommend avoiding the slow presets of the older encoders (x264, x265), as the recent encoders (x265, VVenC) offer higher quality for the same bitrate-energy performance and provide a lower rate for the same energy-distortion performance.

==> name.tex <==
In this work we evaluate the performance of the surface fitting technique using the evaluation metric, mean average percentage error (MAPE). First, and foremost we evaluate the accuracy of the surface fitting techniques based on the supporting points. To do so, we we compute the mean relative error (MAPE) between the distortion values of the intermediate non-supporting points $d_{i}$ and their corresponding fitted values $\hat d_{\mathrm {ns,}i}$ as follows:

we evaluate the 
It is calculated using distortion values of the data points $d_{\mathrm {,}i}$ and their corresponding fitted values $\hat d_{\mathrm {ns,}i}$ as follows: which is defined as follows: \begin{equation} \label{eval}\overline{\epsilon_{\mathrm {t}}}=\frac{1}{N}\sum_{i=1}^{N} \Bigg\vert \frac{\hat d_{\mathrm {t,}i}- d_{\mathrm {t,}i}}{d_{\mathrm {t,}i}} \Bigg\vert, \end{equation}
where t represents the type of data points, 

Similar to, \cite{BB}, in this work, we evaluate the surface fitting techniques, for the supporting points and intermediate non-supporting points.


%In this work, we evaluate the surface fitting techniques, using three evaluation metrics. First, we evaluate the surface fitting techniques based on how well the response values from the surface fitting corresponds to the supporting points using Sum of Squared Errors (SSE). SSE quantifies  the total deviation of the response values from the fit compared to those of the supporting points, and expressed as:
%\begin{equation}\label{SSE}
%SSE=\sum_{i=1}^{n}(d_i-\bar{d_i})^2,
%\end{equation}
%where $d_i$ represents the actual response values from the supporting points, $\bar{d_i}$ represents the predicted response values obtained from the surface fitting, and $n$ denotes the total number of data points. A smaller SSE value indicates that the model exhibits a lesser random error component, implying that the fit is more accurate and potentially more reliable. Secondly, we employed another statistical metric known as R-Square, which assesses the effectiveness of the fit in elucidating the supporting points's variance. Essentially, R-Square represents the square of the correlation between the observed response values and the predicted response values. R-Square ranges between 0 and 1, with values closer to 1 indicating that a larger proportion of the variance in the data is explained by the model. 

Lastly, we assess the surface fitting techniques by evaluating their ability to accurately represent non-supporting intermediate points. To achieve this, we generate a set of $N$ rate-energy-distortion triplets ($r_{\mathrm {ns}}, e_{\mathrm {ns}}, d_{\mathrm {ns}}$) corresponding to intermediate non-supporting points on the surface. Subsequently, we apply the surface fitting techniques to derive the fitted distortion values $\hat d_{\mathrm {ns}}$ for these intermediate non-supporting points based on their rate-energy data. Finally, we compute the mean relative error (MAPE) between the distortion values of the intermediate non-supporting points $d_{\mathrm {ns,}i}$ and their corresponding fitted values $\hat d_{\mathrm {ns,}i}$ as follows:
\begin{equation} \label{eval}\overline{\epsilon}=\frac{1}{N}\sum_{i=1}^{N} \Bigg\vert \frac{\hat d_{\mathrm {ns,}i}- d_{\mathrm {ns,}i}}{d_{\mathrm {ns,}i}} \Bigg\vert, \end{equation}

The MRE (Mean Relative Error) values for surface fitting techniques employed in the study, averaged across all sequences, are presented in Table \ref{tab:accuracy}.


Table \ref{tab:gof} presents the mean SSE and mean R-square values for the surface fitting techniques employed in the study, averaged across all sequences analyzed. The findings highlight the following observations: Linear interpolation emerges as the most effective technique in terms of goodness-of-fit metrics. It achieves a SSE of 0 and an R-square value of 1 for all encoder implementations, indicating that the fit explains 100\% of the total variation in the data about the average. 


%In this section, we present an evaluation of the surface fitting techniques outlined in Section \ref{sec:fitting} and assess its accuracy. First, we evaluate the surface fitting techniques based on how well the response values from the surface fitting corresponds to the supporting points in Section \ref{subsec:gof}. Second, we evaluate accuracy of the surface fitting techniques, based on how well the non-supporting intermediate points are fitted in Section \ref{subsec:accuracy}. Lastly, we use the projection of the fitted surface to make various interpretation of the rate-energy-distortion performance in Section \ref{subsec:gof}.
%In this section, we present an evaluation of the surface fitting techniques described in Section \ref{subsec:fitting} and assess its accuracy. First, we evaluate the surface fitting techniques based on how well the response values from the surface fitting corresponds to the supporting points in \ref{subsec:gof}. Second, we evaluate accuracy of the surface fitting techniques, based on how well the non-supporting intermediate points are fitted in Section \ref{subsec:accuracy}. Lastly, we use the projection of the fitted surface to make various interpretation of the rate-energy-distortion performance in Section \ref{subsec:gof}.
%\subsection{Goodness of the fit}\label{subsec:gof}
%The goodness of fit evaluates the effectiveness of surface fitting techniques by examining the correspondence between the response values derived from the surface fitting and the supporting points.

%One important metric used for this evaluation is the Sum of Squares Due to Error (SSE), which quantifies the total deviation of the response values from the fit compared to those of the supporting points. It is also known as the summed square of residuals. Mathematically, it can be expressed as:
%The Goodness of the fit evaluates the surface fitting techniques based on how well the response values from the surface fitting corresponds to the supporting points. First is the, Sum of Squares Due to Error, a statistic that measures the total deviation of the response values from the fit to that of the supporting points' values as in \eqref{}. It is also called the summed square of residuals and is usually labeled as SSE. A value closer to 0 indicates that the model has a smaller random error component, and that the fit will be more useful for prediction.
%\begin{equation}\label{SSE}
%SSE=\sum_{i=1}^{n}(d_i-\bar{d_i})^2,
%\end{equation}
%where $d_i$ represents the actual response values from the supporting points, $\bar{d_i}$ represents the predicted response values obtained from the surface fitting, and $n$ denotes the total number of data points.A smaller SSE value indicates that the model exhibits a lesser random error component, implying that the fit is more accurate and potentially more reliable. 

%Furthermore, we employed another statistical metric known as R-Square, which assesses the effectiveness of the fit in elucidating the data's variance. Essentially, R-Square represents the square of the correlation between the observed response values and the predicted response values. It is calculated as the ratio of the sum of squares of the regression (SSR) to the total sum of squares (SST) as in \eqref{RSquare}. R-Square ranges between 0 and 1, with values closer to 1 indicating that a larger proportion of the variance in the data is explained by the model.
%\begin{equation}\label{RSquare}
%SSE=\sum_{i=1}^{n}(d_i-\bar{d_i}^2)
%\end{equation}
%In addition, we use another statistic, called R-Square, that measures how successful the fit is in explaining the variation of the data. In other words, R-square is the square of the correlation between the response values and the predicted response values. R-square is defined as the ratio of the sum of squares of the regression (SSR) and the total sum of squares (SST). R-square can take on any value between 0 and 1, with a value closer to 1 indicating that a greater proportion of variance is accounted for by the model. 

Table \ref{tab:gof} presents the mean SSE and mean R-square values for the surface fitting techniques employed in the study, averaged across all sequences analyzed. The findings highlight the following observations: Linear interpolation emerges as the most effective technique in terms of goodness-of-fit metrics. It achieves a SSE of 0 and an R-square value of 1 for all encoder implementations, indicating that the fit explains 100\% of the total variation in the data about the average. 

Following linear interpolation, the polynomial regression equation defined in \eqref{poly32} exhibits notable performance. It yields SSE values of 4.56, 4.32, and 0.07 for x264, x265, and VVenC, respectively. Additionally, for x264, x265, and VVenC, it achieves R-square values of 0.99, 0.99, and 1, respectively, signifying that the fit explains 99\%, 99\%, and 100\% of the total variation in the data. 

Lastly, the polynomial expression derived using \eqref{custom} demonstrates respectable performance, although with higher SSE values compared to the other techniques. For x264, x265, and VVenC, it yields SSE values of 8.92, 6.17, and 0.21, respectively. Additionally, it achieves R-square values of 0.97, 0.99, and 1, respectively, indicating that it explains 97\%, 99\%, and 100\% of the total variation in the data. In summary, the results highlights the the effectiveness of linear interpolation in accurately capturing data variation.
%Table \ref{tab:gof} gives the mean SSE and mean R-square values of the surface fitting techniques used in the study, averaged over all the sequence studied. This table shows that, the linear interpolation is best with respect to goodness of the fit metrics, with Sum of Squares Due to Error being 0, with a R-square value of 1 for all the encoder implementations, which means that the fit explains  100 \%of the total variation in the data about the average. In terms of goodness of the fit metrics, it is followed by the polynomial regression equation defined in \eqref{poly32}, with Sum of Squares Due to Error being 4.56, 4.32, and 0.07 for x264, x265, and VVenC respectively. In addition, \eqref{poly32} has a R-square value of 0.99, 0.99, 1 for for x264, x265, and VVenC respectively, meaning that the fit explains  99\%, 99\%, 100\%of the total variation in the data for x264, x265, and VVenC respectively. That leaves the polynomial expression using \eqref{custom}, has Sum of Squares Due to Error as 8.92, 6.17, and 0.21 x264, x265, and VVenC respectively. In addition, \eqref{custom} has a R-square value indicates that the fit explains  97\%, 99\%, 100\%of the total variation in the data for x264, x265, and VVenC respectively.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Evaluation Metrics -Supporting Points}
\label{tab:gof}
\begin{tabular}{|l|lll|lll|}
\hline
\multirow{2}{*}{Enc Imp} & \multicolumn{3}{c|}{SSE}                                  & \multicolumn{3}{c|}{R-Square}                             \\ \cline{2-7} 
 &
  \multicolumn{1}{l|}{Linear} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Poly. \\ (5)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Poly.\\ (6)\end{tabular} &
  \multicolumn{1}{l|}{Linear} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Poly. \\ (5)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Poly.\\ (6)\end{tabular} \\ \hline
x264                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{4.56} & 8.92 & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{0.99} & 0.97 \\ \hline
x265                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{4.32} & 6.17 & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{0.99} & 0.99 \\ \hline
VVenC                    & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.07} & 0.21 & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{1}    & 1    \\ \hline
\end{tabular}
\end{table}
\subsection{Accuracy}\label{subsec:accuracy}
We assess the accuracy of surface fitting techniques by evaluating their ability to accurately represent non-supporting intermediate points. To achieve this, we generate a set of $N$ rate-energy-distortion triplets ($r_{\mathrm {ns}}, e_{\mathrm {ns}}, d_{\mathrm {ns}}$) corresponding to intermediate non-supporting points on the surface. Subsequently, we apply the surface fitting techniques to derive the fitted distortion values $\hat d_{\mathrm {ns}}$ for these intermediate non-supporting points based on their rate-energy data. Finally, we compute the mean relative error (MRE) between the distortion values of the intermediate non-supporting points $d_{\mathrm {ns,}i}$ and their corresponding fitted values $\hat d_{\mathrm {ns,}i}$ as follows:
%We evaluate accuracy of the surface fitting techniques, based on how well the non-supporting intermediate points are fitted. For this, we generate the $N$ number rate-energy-distortion triplets ($r_{\mathrm {ns}}, e_{\mathrm {ns}}, d_{\mathrm {ns}}$) for intermediate non-supporting points on the surface. And then use the surface fitting techniques to obtain the (fitted-) distortion $\hat d_{\mathrm {ns}}$ for the intermediate non-supporting points rate-energy data points. In the end, we calculate the mean relative error (MRE) between intermediate non-supporting points $d_{\mathrm {ns,}i}$ and fitted intermediate non-supporting points $\hat d_{\mathrm {ns,}i}$ as follows:

\begin{equation} \label{eval}\overline{\epsilon}=\frac{1}{N}\sum_{i=1}^{N} \Bigg\vert \frac{\hat d_{\mathrm {ns,}i}- d_{\mathrm {ns,}i}}{d_{\mathrm {ns,}i}} \Bigg\vert, \end{equation}

The MRE (Mean Relative Error) values for surface fitting techniques employed in the study, averaged across all sequences, are presented in Table \ref{tab:accuracy}. The findings reveal that linear interpolation exhibits the highest accuracy, recording MRE values of 0.24\% and 0.30\% for x264 and x265 encoder implementations, respectively. Following linear interpolation, the polynomial expression referenced by \eqref{poly32} demonstrates relatively lower accuracy, with MRE values of 0.71\% and 0.51\% for x264 and x265 encoder implementations. Lastly, the polynomial expression denoted by equation \eqref{custom} shows lowest accuracy of all the considered surface fitting techniques, with MREs of 0.96\% and 0.60\% for x264 and x265 encoder implementations, respectively. %Table \ref{tab:accuracy} gives the MRE of the surface fitting techniques used in the study, averaged over all the sequences studied. This table shows that, the linear interpolation is the most accurate with a MRE of 0.24\% and 0.30\% for x264 and x265 encoder implementations respectively. This is followed by the polynomial expression \eqref{poly32} with a MRE of 0.71\% and 0.51\% for x264 and x265 encoder implementations respectively. Lastly, the polynomial expression \eqref{custom} with a MRE of 0.96\% and 0.60\% for x264 and x265 encoder implementations respectively.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Evaluation Metrics - Non-Supporting Points}
\label{tab:accuracy}
\begin{tabular}{|l|lll|}
\hline
\multirow{2}{*}{Enc Imp} & \multicolumn{3}{c|}{mean relative error (MRE in \%)}         \\ \cline{2-4} 
 & \multicolumn{1}{l|}{Linear} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Poly. \\ (5)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Poly.\\ (6)\end{tabular} \\ \hline
x264                     & \multicolumn{1}{l|}{0.24} & \multicolumn{1}{l|}{0.71} & 0.96 \\ \hline
x265                     & \multicolumn{1}{l|}{0.30} & \multicolumn{1}{l|}{0.51} & 0.60 \\ \hline
\end{tabular}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.45\textwidth]{proj1.jpg}}
\caption{Project of the Rate-energy-distortion surface fitting shown in Figure \ref{RED_all}. Each point represents the R-E-D triplet, obtained by encoding the "BasketballDrive" for x264 (red surface), x265 (blue surface), and VVenC (green surface) encoders VVenC encoder at a specific preset and QP value.}
\label{RED_proj1}
\end{figure}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.45\textwidth]{proj2.jpg}}
\caption{Projections of the Rate-energy-distortion surface fitting shown in Figure \ref{RED_all}. Each point represents the R-E-D triplet, obtained by encoding the "BasketballDrive" for x264 (red surface), x265 (blue surface), and VVenC (green surface) encoders VVenC encoder at a specific preset and QP value.}
\label{RED_proj2}
\end{figure}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.45\textwidth]{RED_all.jpg}}
\caption{Rate-energy-distortion surface fitting using linear interpolation for the sequence "BasketballDrive". Each point represents the R-E-D triplet, obtained by encoding the "BasketballDrive" for x264 (red), x265 (blue), and VVenC (green) encoders VVenC encoder at a specific preset and QP value.}
\label{RED_all}
\end{figure}

In figure \ref{fig:3D}(a), three Rate-Efficiency-Distortion (R-E-D) surfaces for the sequence "BasketballDrive" are depicted, each corresponding to different video encoders, x264, x265, and VVenC. These surfaces provide a visual representation of the trade-offs between rate, encoding energy, and distortion for three encoders. As one traverses this surface, the coding efficiency remains constant. For instance, when the rate is held constant, an increase in energy is anticipated to yield a gain in quality. Conversely, higher energy consumption would not be deemed efficient without such gains.
By examining projections of three 3-D surfaces, we can gain insights into performance of the encoders across different rate, energy, and distortion scales. Nonetheless, any overlapping areas in the projections of the such 3D surfaces offer valuable insights into the performance and trade-offs between different encoders illustrated. 


The Figures \ref{RED_proj1} depicts the R-E projections obtained from the surfaces are illustrated in Figure \ref{RED_all}. This projection illustrates the array of potential combinations of encoder settings, quality levels, and presets necessary to achieve a specific target quality. For a certain target quality, moving up in figure offers better rates with more energy consumption, and moving down offers the better energy with increased rates. In addition, this projection, offers the possibility to select the encoder-quality levels-presets combination for a rate and energy requirements for any given quality. The Overlapping regions indicate areas where the three encoders perform similarly in terms of rate, efficiency, and distortion can be defined as similar performance regions. This suggests that under those specific conditions, the choice of encoder may not significantly impact the outcome. However, when combined with preset and quality level combination one can achieve either rate or energy savings.

The Figures \ref{RED_proj2} depicts the E-D projections obtained from the surfaces are illustrated Figure \ref{RED_all}. This projection illustrates the array of potential combinations of encoder settings, quality levels, and presets necessary to achieve a specific target rate. For a certain target rate, moving right in figure offers better quality with more energy consumption, and moving left offers the better energy with dip in quality. The Overlapping regions indicate areas where the three encoders perform similarly in terms of rate, efficiency, and distortion can be defined as similar performance regions. This suggests that under those specific conditions, the choice of encoder may not significantly impact the outcome. However, when combined with preset and quality level combination one can achieve either improved quality or energy savings.


%The primary objective of traditional video coding is to encode video content with the lowest possible bitrate while maintaining minimal distortion. Distortion is assessed objectively and subjectively. Although PSNR is commonly used, it does not always consistently align with perceived quality \cite{HuynhThu2008}, prompting subjective evaluations which are resource-intensive. Objective measures like SSIM \cite{SSIM}  and VMAF \cite{VMAF} , inspired by HVS, offer efficient approximations of subjective assessments. Since the standardization of the first video codec \cite{}, the term bitrate has been used to describe the transmission or storage requirements of a coded video. Despite the ideal goal of video coding with the lowest possible bitrate and minimal distortion, it is impossible to simultaneously minimize both rate and distortion. Achieving better quality (less distortion) necessitates a higher bitrate to convey all details, while aiming for a lower bitrate results in higher distortion. Therefore, a trade-off between bitrate and distortion is characterized by rate-distortion (R-D) curve fitting.

%During the development of the H.264/AVC video coding standard, a coding efficiency metric called Bjøntegaard-Delta (BD) metric \cite{Bjoentegaard01} was introduced. Proposed by Gisle Bjøntegaard, BD metric employs a third-order logarithmic polynomial to model the bitrate versus PSNR performance and approximate a given rate-distortion (R-D) curve. This metric proves effective in quantifying the average difference between two R-D curves \cite{BB}, providing a robust evaluation of R-D performance. As a result, BD metric serves as an coding efficiency evaluation metric, and it is widely used in video coding research. 


%However, BD metric does not account for energy demand of the encoders. Notably, modern codecs provide a plethora of compression methods, increasing the encoders' processing complexity \cite{VVCComplexity}, resulting in a considerable increase in the energy demand. This substantial energy increase presents a significant challenge for practical video applications, particularly those on servers and handheld devices with energy constraints \cite{Carroll13}. Though, the BD metric has been instrumental in evaluating coding efficiency, there's a pressing need to consider energy efficiency alongside traditional performance metrics. With the rising importance of energy-aware video coding and the need for comprehensive evaluation metrics that encompass both coding and energy efficiency aspects.


%Quality assessment serves to quantify this distortion. It typically falls into two categories: objective measures and subjective measures. Objective measures, such as peak signal-to-noise ratio (PSNR), are commonly utilized but may not consistently correlate with perceptual quality \cite{HuynhThu2008}. As a result, subjective evaluations, which rely on human perception, are employed to assess visual quality. However, these subjective assessments are impractical and time-consuming. To bridge this gap, objective measures adapted from the human visual system (HVS), such as structural similarity (SSIM) \cite{SSIM} and Video Multimethod Assessment Fusion (VMAF) \cite{VMAF}, have been introduced to approximate subjective assessments. 
%The main goals of the traditional video coding is to encode the video with lowest possible rate with very low distortion. The quality assessment gives a measure of distortion. The quality assessment typically falls into two categories: objective measures and subjective measures. Objective measures, such as mean squared error and resulting PSNR, are commonly used but may not always correlate well with perceptual quality [1]. Consequently, subjective evaluations, which rely on human perception, are employed to evaluate visual quality. However, these subjective assessment are impractical and time consuming. To bridge this gap, HVS adapted objective measures, like structural distortion (SSIM), VMAF, have been introduced to approximate subjective assessments. Since the standardization of the first video codec, the term bitrate is used to describe the tramission  or storage requirements of a coded video. Even though, the ideal goal of the video codec, is to code the video with lowest possible rate with very low distortion, it is impossible to minimize the both rate and distortion at the same time. Because for a better quality (less distortion), a higher rate is requires to covey all the details, on the other hand, if the lower rate is expected, the distortion will be higher. Hence, a trade-off between the rate and distortion is characterized by rate-distortion (R-D) curve fitting. Therefore, while the BD metric has been instrumental in evaluating coding efficiency, there's a pressing need to consider energy efficiency alongside traditional performance metrics. With the rising importance of energy-aware video coding and the need for comprehensive evaluation metrics that encompass both coding and energy efficiency aspects. To address this challenge, research has focused on resource and complexity-constrained video coding [7–13]. Consequently, there is a growing need for an objective coding efficiency metric that accounts for complexity. Therefore, this paper proposes a method that integrates complexity considerations into the evaluation of coding efficiency.The proposed method, as an extension of BDPSNR, effectively captures the average difference between two rate-complexity-distortion (R-C-D) surfaces. This enables a fair comparison of coding efficiency among different algorithms with varying complexities.
%\section{Literature Review}
%\subsection{Maintaining the Integrity of the Specifications}
%\section{Rate-Distortion-Energy representation}\label{sec:3D}

%The MAPE values for surface fitting techniques employed in the study, for supporting and non-supporting points, averaged across all sequences, are presented in Table \ref{tab:accuracy}. The findings reveal that linear interpolation exhibits the highest accuracy, recording MAPE values of 0\% based on supporting points for all encoders, 0.24\% and 0.30\% based on non-supporting points for x264 and x265 encoder implementations, respectively. Following linear interpolation, the polynomial expression referenced by \eqref{poly32} demonstrates relatively lower accuracy, with MAPE values of 0.70\%, 0.48\% and 0.11\% based on supporting points for x264, x265, and VVenC encoder implementations and with MAPE of 0.71\% and 0.51\% based on non-supporting points for x264 and x265 encoder implementations. Lastly, the polynomial expression denoted by equation \eqref{custom} shows lowest accuracy of all the considered surface fitting techniques, with MAPE of 1\%, 0.35\%, 0.09\% based on supporting points for x264, x265, and VVenC encoder implementations, and with MAPE of 0.96\% and 0.60\% based on non-supporting points for x264 and x265 encoder implementations, respectively.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{}
\label{tab:accuracy}
\begin{tabular}{|l|llllll|}
\hline
\multirow{3}{*}{\textbf{Enc Imp}} & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Mean absolute percentage error,}\\ (MAPE \%)\end{tabular}}                                      \\ \cline{2-7} 
                         & \multicolumn{3}{l|}{\textbf{supporting points, ${\epsilon_\mathrm{s}}$}}                                         & \multicolumn{3}{l|}{\textbf{non-supporting points, ${\epsilon_\mathrm{ns}}$}}                   \\ \cline{2-7} 
 &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular} \\ \hline
\textbf{x264}                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.70} & \multicolumn{1}{l|}{1}    & \multicolumn{1}{l|}{0.24} & \multicolumn{1}{l|}{0.71} & 0.96 \\ \hline
\textbf{x265}                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.35} & \multicolumn{1}{l|}{0.30} & \multicolumn{1}{l|}{0.51} & 0.60 \\ \hline
\textbf{VVenC}                    & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.11} & \multicolumn{1}{l|}{0.09} & \multicolumn{1}{l|}{-}    & \multicolumn{1}{l|}{-}    & -    \\ \hline
\end{tabular}
\end{table}
%For evaluation, we use the mean absolute percentage error (MAPE), which is an indicator of performance that measures the absolute error between actual and predicted data points in percentage terms, as follows:
%\begin{equation} \label{eval}\overline{\epsilon}=\frac{1}{N_t}\sum_{i=1}^{N_t} \Bigg\vert \frac{\hat d_{t\mathrm {,}i}- d_{t\mathrm {,}i}}{d_{t\mathrm {,}i}} \Bigg\vert, \end{equation}
%where $N_t$ is the number of data points, $t$ here represents the type of data points, as supporting (s) or non-supporting (ns) data points, $\hat d_{t\mathrm {,}i}$ is the distortion predicted by the surface fitting  mentioned in Section \ref{sec:fitting}, $d_{t\mathrm {,}i}$ is the actual distortion recorded during encoding. Firstly, we evaluate the, the performance of the surface fitting techniques based on how well it fits the supporting points. Secondly, we evaluate the performance of the surface fitting techniques, how well fitting happens for non-supporting (ns) data points.
%(a) Rate-energy-distortion surface fitting using linear interpolation for the sequence "BasketballDrive", (b) Projection of the Rate-energy-distortion surface  on R-E plane doe all the encoders. Each point represents the R-E-D triplet, obtained by encoding the "BasketballDrive" for x264 (red surface), x265 (blue surface), and VVenC (green surface) encoders VVenC encoder at a specific preset and QP value. In all these figures, the x264 surface is depicted using red, and supporting points are in green, the x265 surface is depicted using blue, and supporting points are in yellow-brown, and  the VVenC surface is depicted using green, and supporting points are in black.

%The Bjøntegaard Delta rate (BD-rate) objectively assess the coding efficiency of video codecs by analyzing the rate-distortion (R-D) performance. While BD-rate offers valuable insights into R-D performance, it overlooks the encoding energy. In practical video applications, especially for those on handheld devices, it's imperative to consider encoding energy alongside rate and distortion for a comprehensive performance evaluation. Although R-D analysis can be extended to incorporate encoding energy as energy-distortion (E-D), it fails to integrate all three parameters seamlessly. This work proposes a novel approach to address this limitation by introducing a 3-dimensional representation of rate, encoding energy, and distortion through surface fitting. In addition, we evaluate various surface fitting techniques based on their interpolation efficiency. Furthermore, we investigate the proposed 3D representation and its projections. One notable observation is that overlapping regions within the projections provide valuable insights into selecting encoders for enhanced rate-energy-distortion performance. The overlapping areas in projections indicate that the slow presets of the older encoders (x264, x265) should be avoided, as the recent encoders (x265, VVenC) offer a higher quality for the same bitrate-energy performance and provide a lower rate for the same energy-distortion performance.
%In our study, first we measure the encoding energy for various presets and three different encoder implementations. Then, we explore various surface fitting techniques to assess their effectiveness in accurately capturing the relationships between rate, encoding energy, and distortion. Additionally, we offer interpretations derived from the proposed 3D representation, shedding light on the interplay between these parameters and their implications for video coding efficiency. By introducing this innovative approach, we seek to advance the field of video coding evaluation by offering a more comprehensive and nuanced perspective that extends beyond traditional R-D analysis. Our findings have the potential to inform the development of more sophisticated coding algorithms and optimization strategies tailored to address the complex inter dependencies between rate, encoding energy, and distortion in video coding systems.

%As in \cite{Herglotz18c}, we describe the energy demand of the encoding process using two consecutive measurements. First, the total energy consumed $E_{\mathrm {total}}$ during the encoding process for the duration of the encoding process $T$ and then, the energy consumed in idle mode $E_{\mathrm {idle}}$ over the same encoding duration $T$. Ultimately, the encoding energy $E_{\mathrm {enc}}$ is the difference between these two measurements as in \eqref{ee}.

%Analogous to the convexity property of the R-D function, it can be further demonstrated that the R-E-D function is also convex. Based on this, D(R, E) can be fitted by proper functions, we assume that D(R, E) can be approximated by the \eqref{custom}. 

%Figure \ref{fig}, shows an example of the surface fitting using linear interpolation for the class B sequence "BasketballDrive", where data points (blue circles) represents the R-E-D triplet obtained by encoding the sequence at different QPs {22, 27, 32, 37} (top to bottom) and different presets $\textit{faster}$, $\textit{fast}$, $\textit{medium}$, $\textit{slow}$, $\textit{slower}$ (right to left), VVenC encoder.
\begin{table}[]
\centering
\caption{Evaluation metric MAPE for supporting points and non-supporting points.}
\label{tab:accuracy}
\begin{tabular}{|l|llllll|}
\hline
\multirow{3}{*}{\textbf{Enc Imp}} & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Mean absolute percentage error,}\\ (MAPE \%)\end{tabular}}                                      \\ \cline{2-7} 
                         & \multicolumn{3}{l|}{\textbf{supporting points, ${\epsilon_\mathrm{s}}$}}                                         & \multicolumn{3}{l|}{\textbf{non-supporting points, ${\epsilon_\mathrm{ns}}$}}                   \\ \cline{2-7} 
 &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular} \\ \hline
\textbf{x264}                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.70} & \multicolumn{1}{l|}{1}    & \multicolumn{1}{l|}{0.24} & \multicolumn{1}{l|}{0.71} & 0.96 \\ \hline
\textbf{x265}                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.35} & \multicolumn{1}{l|}{0.30} & \multicolumn{1}{l|}{0.51} & 0.60 \\ \hline
\textbf{VVenC}                    & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.11} & \multicolumn{1}{l|}{0.19} & \multicolumn{1}{l|}{-}    & \multicolumn{1}{l|}{-}    & -    \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Evaluation metric MAPE for supporting points ${\epsilon_\mathrm{s}}$ and non-supporting points ${\epsilon_\mathrm{ns}}$.}
\label{tab:accuracy}
\begin{tabular}{|l|llllll|}
\hline
\multirow{3}{*}{\textbf{Enc Imp}} & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Mean absolute percentage error,}\\ (MAPE \%)\end{tabular}}                                      \\ \cline{2-7} 
                         & \multicolumn{3}{l|}{\textbf{supporting points, ${\epsilon_\mathrm{s}}$}}                                         & \multicolumn{3}{l|}{\textbf{non-supporting points, ${\epsilon_\mathrm{ns}}$}}                   \\ \cline{2-7} 
 &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{Linear}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Poly}. \\ \eqref{poly32}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}\textbf{Poly}.\\ \eqref{custom}\end{tabular} \\ \hline
x264                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.27} & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.27} & \multicolumn{1}{l|}{0.92} & 1.16 \\ \hline
x265                     & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.17} & \multicolumn{1}{l|}{0.26} & \multicolumn{1}{l|}{0.32} & \multicolumn{1}{l|}{0.72} & 0.84 \\ \hline
VVenC                    & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0.11} & \multicolumn{1}{l|}{0.19} & \multicolumn{1}{l|}{-}    & \multicolumn{1}{l|}{-}    & -    \\ \hline
\end{tabular}
\end{table}
%However, PSNR may not consistently align with perceived quality \cite{HuynhThu2008}, necessitating resource-intensive subjective assessments. Objective measures like structural similarity (SSIM) \cite{SSIM} and video multimethod assessment fusion (VMAF) \cite{VMAF} offer efficient approximations inspired by the human visual system (HVS). Bitrate is the term that has been used to describe transmission or storage requirements since the standardization of the first video codec \cite{}. Despite the goal of video coding being to obtain the lowest possible bitrate and minimal distortion, it is impossible to simultaneously minimize both rate and distortion. Therefore, a trade-off between bitrate and distortion is characterized by rate-distortion (R-D) curve fitting.
